Norms on Categories and Analogs of the Schr\"oder-Bernstein Theorem

We generalize the concept of a norm on a vector space to one of a norm on a category. This provides a unified perspective on many specific matters in many different areas of mathematics like set theory, functional analysis, measure theory, topology, and metric space theory. We will especially address the two last areas in which the monotone-light factorization and, respectively, the Gromov-Hausdorff distance will naturally appear. In our formalization a Schr\"oder-Bernstein property becomes an axiom of a norm which constitutes interesting properties of the categories in question. The proposed concept provides a convenient framework for metrizations.

==> introduction/notation_Thickenings.tex <==
\subsection{Norms and metrics}\label{ssec:norms_metrics}

\begin{itemize}
    \item norms $\Norm{}{foo}[bar]$ on categories, e.g.\ vector spaces.
    \item specific norms: 
        $ \abs{(r_1, \ldots, r_{\dim})} \coloneqq \abs{r_1} \vee \ldots \vee \abs{r_{\dim}} $,
        $ \abs{f} \coloneqq \sup_{x \in X} \abs{f(x)} $ for $ f\colon X \to \R^{\dim}$.
        As well as $
                \abs{(r_1, \ldots, r_{\dim})}_p
            \coloneqq
                \sqrt[p]{r_1^p + \ldots + r_{\dim}^p }
        $ and $ 
            \abs{f}_p \coloneqq \sup_{x \in X} \abs{f(x)}_p 
        $ for $ f\colon X \to \R^{\dim}$.
    \item Define the thickenings 
        \begin{align*}
            A^{r)} &\coloneqq \bigcup_{x \in A} \Openball{x}{r} 
        \intertext{for $r>0$ and for $r\geq 0$}
            A^{r]} &\coloneqq \bigcap_{r' > r} A^{r')}
        \end{align*}

        Note $A^{r]}$ closed since $\bigcap_{r' > r} A^{r')} \supset \bigcap_{r' > r} \overline{A^{r'/2)}} = \bigcap_{r' > r} \overline{A^{r')}}  $. Further
        \begin{align*}
            A^{0)} &\coloneqq A^{\circ}
        \\
                A^{-r)} 
            &\coloneqq
                A^{\mathrm{C}\; r]\; \mathrm{C}}
            =
                \left(\bigcap_{r' > r} A^{\mathrm{C}\; r']}\right)^{\mathrm{C}}
            =
                \bigcup_{r' > r} A^{\mathrm{C}\; r']\;\mathrm{C}}
        \\
                A^{-r]} 
            &\coloneqq
                A^{\mathrm{C}\; r)\; \mathrm{C}}
            =
                \left(\bigcup_{x \in A} \Openball{x}{r} \right)^{\mathrm{C}}
            =
                \bigcup_{x \in A} \Openball{x}{r}^{\mathrm{C}}
        \end{align*}
        \todo{the negative thickenings are actually so far not needed}
        \begin{subequations}
            For $ r \geq 0 $ and $s > 0$ note the inclusions
            \begin{equation}
            \label{eq:openThickeningIncl}
                A^{r)\;s)}, A^{r]\;s)} \subset A^{r+s)}
            \end{equation}
            that hold since
            \begin{align*}
                    A^{r)\;s)} \subset A^{r]\;s)} 
                &=
                    \left( \bigcap_{r' > r} A^{r')} \right)^{s)}
            \\
                &=
                    \setBuilder*
                      {y\in X}
                      {\exists x \in \bigcap\nolimits_{r' > r} A^{r')} \colon \dist{x}{y} < s}
            \\
                &=
                    \setBuilder*
                      {y\in X}
                      {\exists z \in A \colon \dist{x}{z} < s}
            \\
                &=
                    A^{r+s)}
            \text{.}
            \end{align*}
            Further note the inclusion
            \begin{equation}
            \label{eq:closedThickeningIncl}
                A^{r]\;s]}, A^{r]\;s]} \subset A^{r+s]}
            \end{equation}
            for $r,s \geq 0$ that holds due to
            \begin{equation*}
                    A^{r)\;s]} \subset A^{r]\;s]} 
                =
                    \bigcap_{s' > s} A^{r]\; s')}
            %\\
                \stackrel{\cref{eq:openThickeningIncl}}{\subset}
                    \bigcap_{s' > s + r} A^{s')}
            %\\
                =
                    A^{r+s]}
            \text{.}
            \end{equation*}
        \end{subequations}
        
    \item set theoretic complement $A^{\mathrm{C}} \coloneqq \spSet \setminus A$.
    \item 
        $ \configurations[n](X) \coloneqq \setBuilder{(x_1,\ldots,x_n)\in X^{\times n}}{x_1, \ldots, x_n \text{ are pairwise distinct} } $
    \item Let $f\colon \spSp \to \spSp*$ be a map of pqmetric spaces. We define the \definiendum{pullback metric} as $
        f^*\spMet*(x,y) \coloneqq \dist{f(x)}{f(y)}_{\spSp*}
    $. Note that the pullback of a metric may be a qmetric.
    The map $f$ is an \definiendum{embedding} if $f^*\spMet* = \spMet$.
\end{itemize}

\color{black}
